Characterising SMSS J2157--3602, the most luminous known quasar, with accretion disc models

We develop an accretion disc (AD) fitting method, utilising thin and slim disc models and Bayesian inference with the Markov-Chain Monte-Carlo approach, testing it on the most luminous known quasar, SMSS J215728.21-360215.1, at redshift $z=4.692$. With a spectral energy distribution constructed from near-infrared spectra and broadband photometry, the AD models find a black hole mass of $\log(M_{\rm{AD}}/M_{\odot}) = 10.31^{+0.17}_{-0.14}$ with an anisotropy-corrected bolometric luminosity of $\log{(L_{\rm{bol}}/\rm{erg\,s^{-1}})} = 47.87 \pm 0.10$, and derive an Eddington ratio of $0.29^{+0.11}_{-0.10}$ as well as a radiative efficiency of $0.09^{+0.05}_{-0.03}$. Using the near-infrared spectra, we estimate the single-epoch virial black hole mass estimate to be $\log(M_{\rm{SE}}/M_{\odot}) = 10.33 \pm 0.08$, with a monochromatic luminosity at 3000\AA\ of $\log{(L(\rm{3000\text{\AA}})/\rm{erg\,s^{-1}})} = 47.66 \pm 0.01$. As an independent approach, AD fitting has the potential to complement the single-epoch virial mass method in obtaining stronger constraints on properties of massive quasar black holes across a wide range of redshifts.

==> backup.tex <==
\begingroup
\begin{table}
\caption {\label{tab:J2157_photometry} Crossmatched photometric information obtained for J2157-3602.}  
\begin{tabular}{lccc}
\hline \hline
 Survey & Filter & Magnitude & Zero-point\\ 
 & ($\mu$m) & (mag) & (Jy) \\ \hline
 Gaia DR3 & bp (0.532) & $19.844 \pm 0.054$ & 3478.8\\
 & g (0.673) & $18.265 \pm 0.003$ & 2861.3\\
 & rp  (0.797) & $17.105 \pm 0.009$ & 2461.22\\
 \hline
 SMSS DR3 & g (0.503) & $20.21 \pm 0.01$ & 3631\\ 
 & r (0.610) & $18.82 \pm 0.01$ & 3631\\ 
 & i (0.775) & $17.29 \pm 0.01$ & 3631\\ 
 & z (0.912) & $17.07 \pm 0.01$ & 3631\\ 
 \hline
 NSC DR2 & g (0.4808) & $20.828 \pm 0.024$ & 3631 \\
 & i (0.7815) & $17.297 \pm 0.004$ & 3631\\
 & z (0.9169) & $17.107 \pm 0.004$ & 3631\\
 \hline
 2MASS & J (1.235)& $15.70 \pm 0.06$ & 1594\\
 & H (1.662) & $14.84 \pm 0.05$ & 1024\\
 & K$_{\rm{s}}$ (2.159) & $14.16 \pm 0.06$ & 666.7\\
 \hline
 VHS DR6 & J (1.252) & $15.639 \pm 0.006$ & 1545\\
 & K$_{\rm{s}}$ (2.147) & $14.214 \pm 0.007$ & 670\\
 \hline
 ALLWISE & W1 (3.35) & $13.11 \pm 0.02$ & 309.54\\
 & W2 (4.6) & $12.60 \pm 0.03$ & 171.787\\
 & W3 (11.56) & $9.91 \pm 0.05$ & 31.674\\
 & W4 (22.1) & $7.42 \pm 0.10$ & 8.363\\

\hline \hline
\end{tabular}
\end{table}
\endgroup
